Generalized Integer Splines on Arbitrary Graphs

Generalized integer splines on a graph $G$ with integer edge weights are integer vertex labelings such that if two vertices share an edge in $G$, the vertex labels are congruent modulo the edge weight. We introduce collapsing operations that reduce any simple graph to a single vertex, carrying with it the edge weight information. This corresponds to a sequence of surjective maps between the associated spline modules, leading to an explicit construction of a module basis in terms of the edge weights.

==> extras.tex <==
Removed from original, may need later.


We note two important corollaries of Theorem\ref{theorem:CRT}.
\begin{corollary}
\label{corr:GCD of moduli}
Suppose
\begin{align*}
    x_{0}   &\equiv x_{1} \bmod m_{1}\\
    x_{1}   &\equiv x_{2}   \bmod m_{2}\\
        &\vdots\\
    x_{k-1} &\equiv x_{k} \bmod m_{k}
\end{align*}
This system of congruences has a solution if and only if $$x_{0} \equiv x_{k} \bmod (m_{1}, m_{2}, \ldots, m_{k}).$$
\end{corollary}
\begin{proof}
We prove this by induction on $m_{k}$.  

If $n = 2$, we have
\begin{align*}
    x_{0}   &\equiv x_{1} \bmod m_{1}\\
    x_{1}   &\equiv x_{2}   \bmod m_{2}
\end{align*}
Equivalently,
\begin{align*}
    x_{1}   &\equiv x_{0} \bmod m_{1}\\
    x_{1}   &\equiv x_{2}   \bmod m_{2}
\end{align*}
so by Theorem \ref{theorem:CRT}, this system is solvable if and only if $x_{0} \equiv x_{2} \bmod (m_{1}, m_{2})$.

Suppose the statement is true for $n = k$.  Consider the system
\begin{align*}
    x_{0}   &\equiv x_{1} \bmod m_{1}\\
    x_{1}   &\equiv x_{2}   \bmod m_{2}\\
        &\vdots\\
    x_{k-1} &\equiv x_{k} \bmod m_{k}\\
    x_{k}   &\equiv x_{k+1} \bmod m_{k+1}
\end{align*}
Since the statement is true for $n = k$, then a solution exists if and only if
\begin{align*}
    x_{0}   &\equiv x_{k}   \bmod (m_{1}, m_{2}, \ldots, m_{k})
\end{align*}
But we must also have $x_{k+1} \equiv x_{k} \bmod m_{k+1}$.  Consequently, by Theorem \ref{theorem:CRT}, $x_{0} \equiv x_{k+1} \bmod ( (m_{1}, m_{2}, \ldots,m_{k}), m_{k+1})$.

But $( (m_{1}, m_{2}, \ldots,m_{k}), m_{k+1}) = ( m_{1}, m_{2}, \ldots,m_{k}, m_{k+1})$.

Hence if the statement is true for $n = k$, it is true for $n = k+1$, which completes the induction.
\end{proof}
In addition:
\begin{corollary}
\label{corr:LCM of moduli}
Suppose
\begin{align*}
    x   &\equiv a \bmod m_{1}\\
    x   &\equiv a \bmod m_{2}\\
        &\vdots\\
    x   &\equiv a \bmod m_{n}\\        
\end{align*}
This system of congruences has solution if and only if $x \equiv a \bmod [m_{1}, m_{2}, \ldots, m_{n}]$.
\end{corollary}


{\textbf{Notation:}} 
\begin{itemize}
\item Let  $G-{v}$ denote the deletion of vertex $v$ and its incident edges but not the adjacent vertices. 
\item Let $G\backslash e$ denote the deletion of the edge $e$.
\item 
\end{itemize}

\begin{figure}
\begin{center}
\begin{tabular}{ccc}
\includegraphics[scale=0.3]{starclique1}
    &$\raisebox{1in}{\longrightarrow}$
        &\includegraphics[scale=0.3]{starclique2}
\end{tabular}
\end{center}
\caption{Star-Clique Operation on $v_4$}
\label{fig:starclique}
\end{figure}



Let $(G,A)$ be a connected simple graph and let $v$ be a vertex of degree $d$ in $G$.  The {\textbf{star-clique}} operation with respect to vertex $v$ converts $G$ to $G_v$ as follows.  
\begin{enumerate}
\item Let $G_v = G$. 
\Remove $v$ and its incident edges from $G_v$.
\item For each path of the form $xvy$ in $G$ with edge weights $a$ and $b$, add an edge $xy$ to $G_v$ with weight $(a,b)$.
\item Leave all the other vertices and edges the same.
  \end{enumerate}
  
  We define $(G_v,A_v)$ more formally below.
  
  \begin{definition}  Let $(G,A)$ be a connected simple graph and let $v$ be a vertex of degree $d$ in $G$, with adjacent vertices  $v_1,\ldots,v_d$ and incident edge weights $a_1,\ldots,a_d$.  The {\textbf{star-clique}} operation with respect to vertex $v$ takes $(G,A)$ to $(G_v,A_v)$ as follows. 
  \begin{enumerate}
    \item $G_v = (G - v )\cup \{e_{ij} : 1 \leq i \leq j \leq d\}$, where $e_{ij }$ is a new edge between $v_i$ and $v_j$.
    \item $A_v(e_{ij}) = (a_i,a_j)$, for all  $1 \leq i \leq j \leq d $.
    \item  $A_v(e) = A(e)$  for any edge $e$ in $G$ not incident to $v$.
\end{enumerate}
\end{definition}
(see Figure \ref{fig:starclique}).  

%Since $G$ is connected, every vertex has degree at least $1$.  If  $G$ is not %$K_{2}$,  then any vertex of degree 1 is adjacent to a vertex of degree at least 2.
Notice that although $G$ is simple, $G_v$ may have multiple edges.  Also note that $G_v$ will have one fewer vertex than $G$, but may have more edges.


We now define an \textbf{edge collapse} operation, in order to reduce multiple edges between two vertices to a single edge.

\begin{definition} Let $(G,A)$ be an edge weighted graph.
Let vertices $v_1, v_2$ be joined by edges $e_1$ and $e_2$ with weights $a$ and $b$.  In an \textbf{edge collapse}, $e_1$ is deleted and the edge weight of $e_2$ is replaced with $[a, b]$.  We define $(G_{e_1},A_{e_1})$ by 
\begin{enumerate}
\item $G_{e_1} = G \backslash {e_1} $  
\item $A_{e_1}(e_2)=[a, b]$ 
\item $A_{e_1}(e)=A(e)$ for all other edges in $G_{e_1}$. 
\end{enumerate}
\end{definition}


For the \textbf{edge collapse operation}, we need the following:
\begin{lemma}
\label{lemma:LCM of GCD}
$[(e_{1}, e_{2}, \ldots, e_{n}, a), (e_{1}, e_{2}, \ldots, e_{n}, b)] = [(e_{1}, e_{2}, \ldots, e_{n}, [a, b])]$
\end{lemma}
\begin{proof}
Let $p$ be prime, and let $p^{k}$ be a divisor of $[(e_{1}, e_{2}, \ldots, e_{n}, a), (e_{1}, e_{2}, \ldots, e_{n}, b)]$.  Then $p^{k}$ must divide either $(e_{1}, e_{2}, \ldots, e_{n}, a)$ or $(e_{1}, e_{2}, \ldots, e_{n}, b)$.  Consequently $p^{k}$ must divide $e_{1}, e_{2}, e_{n}, \ldots$, and either $a$ or $b$, so $p^{k}$ divides $[a, b]$, and so $p^{k}$ divides $[(e_{1}, e_{2}, \ldots, e_{n}, [a, b])]$.

Conversely, let $p^{k}$ be a prime divisor of $[(e_{1}, e_{2}, \ldots, e_{n}, [a, b])]$. Therefore, it must divide $e_{1}$, $e_{2}$, \ldots, $e_{n}$, and $[a, b]$.  Since $p$ is prime, $p^{k}$ must divide either $a$ or $b$; we assume $p^{k}$ divides $a$.  Consequently $p^{k}$ divides $(e_{1}, e_{2}, \ldots, e_{n}, a)$.  But $(e_{1}, e_{2}, \ldots, e_{n}, a)$ is a divisor of $[(e_{1}, e_{2}, \ldots, e_{n}, a), (e_{1}, e_{2}, \ldots, e_{n}, b)]$.  Consequently $p^{k}$ divides
$[(e_{1}, e_{2}, \ldots, e_{n}, a), (e_{1}, e_{2}, \ldots, e_{n}, b)]$.
\end{proof}



We begin with a star clique, removing vertex $D$ and joining the neighbors of $D$ with an edge having weight $(9, 12) = 3$ (Figure \ref{fig:collapse}a).



Now $B$, $E$ are joined by two edges.  These may be replaced by edge deletion with a single edge, having weight $[10, 3] = 30$ (Figure \ref{fig:collapse}b). 

Now we remove vertex $C$ by star collapse.  Since vertices $A$, $E$ are joined to $C$ by paths of weight $9, 3$, we add an edge between $A$, $E$, with a weight of $(9, 3) = 3$.  Similarly we add an edge between $A$, $B$ of weight $(9, 6) = 3$; and an edge between $B, E$ of weight $(3, 6) = 3$ (Figure \ref{fig:collapse}c). 



We replace the two edges between $A, B$ with a single edge of weight $[3, 8] = 24$; the edges between $B$, $E$ with a single edge of weight $[30,3] = 30$; and the edge between $A$, $E$ with a single edge of weight $[14, 3] = 42$ (Figure \ref{fig:collapse}d through \ref{fig:collapse}g).

We remove vertex $E$ by a star collapse, connecting its neighbors $A, B$ with a vertex of weight $(42, 30) = 6$ (Figure \ref{fig:collapse}h).

Finally $A, B$ are joined by two edges, so these can be replaced by a single edge with weight $[24, 6] = 24$ (Figure (Figure \ref{fig:collapse}i).

The sequence of deleted vertices gives the collapse ordering $\left\{A, B, E, C, D\right\}$.

Now suppose we wish to produce a spline $(x_{A}, x_{B}, x_{E}, x_{C}, x_{D})$.  We choose $x_{A} = 3$ arbitrarily.  Then $x_{B} \equiv 3 \bmod 24$, so $x_{B} = 27$ is a nontrivial solution.  Note that the assignment $x_{A} = 3$, $x_{B} = 27$ also satisfies the edge-weighted graph in Figure \ref{fig:collapse8}.

To find $x_{E}$, we note it must satisfy
\begin{align*}
    x_{E}   &\equiv     3 \bmod 42\\
    x_{E}   &\equiv     27 \bmod 30
\end{align*}
Since $3 \equiv 27 \bmod (42, 30)$, such a value  exists: the least such value is $x_{E} = 87$, and note the assignment $x_{A} = 3$, $x_{B} = 27$, $x_{E} = 87$ also satisfies the edge weighted graphs of  Figures \ref{fig:collapse5},  \ref{fig:collapse4}, and  \ref{fig:collapse3}.

To find $x_{C}$, we note that it must satisfy the congruences
\begin{align*}
    x_{C}   &\equiv 3 \bmod 9\\
    x_{C}   &\equiv 27 \bmod 6\\
    x_{C}   &\equiv 87 \bmod 3
\end{align*}
which can be reduced to
\begin{align*}
    x_{C}   &\equiv 3 \bmod 9\\
    x_{C}   &\equiv 3 \bmod 6\\
    x_{C}   &\equiv 0 \bmod 3
\end{align*}
which has least solution $x_{C} = 3$.  We reject this value as uninteresting.  The next possibility is $21$, so we take $x_{C} = 21$.  Again, this assignment also satisfies the edge weighted graph of Figure \ref{fig:collapse1}. 

It remains to find $x_{D}$ that satisfies the original edge weighted graph.  We note that
\begin{align*}
    x_{D}   &\equiv 27 \bmod 12\\
    x_{D}   &\equiv 87 \bmod 9
\end{align*}
which reduces to
\begin{align*}
    x_{D}   &\equiv 3 \bmod 12\\
    x_{D}   &\equiv 6 \bmod 9
\end{align*}
which yields $x_{D} = 15$ as a solution.

This gives the spline $(x_{A}, x_{B}, x_{E}, x_{C}, x_{D}) = (3, 27, 87, 21, 15)$.

\section{Paths to Zero}

Of particular interest are the so-called \textbf{paths to zero}.  To introduce these, we recall the following ideas from graph theory:
\begin{definition}
Let $G$ be a graph with vertex set $V$ and edge set $E$.  A \textbf{path in $G$} is a sequence of vertices and edges $\mathcal{P} = \left\{p_{0}, e_{1}, p_{1}, e_{1}, \ldots, e_{n} p_{n}\right\}$ such that $p_{i} \neq p_{j}$ for $i \neq j$.  
\end{definition}
We say that $\mathcal{P}$ is a path from $p_{0}$ to $p_{n}$, and we say the vertices $p_{1}$, $p_{2}$, \ldots, $p_{n-1}$ are the intermediate vertices.  Note that we are allowing the possibility for multiple edges to join two vertices; hence the necessity of specifying both the vertices and the edges along the path.  
\begin{definition}
Let $\mathcal{P}$ be a path in $(G, A)$, along edges $e_{p_{1}}$, $e_{p_{2}}$, \ldots, $e_{p_{n}}$.  We define $W(\mathcal{P}) = (a_{p_{1}}, a_{p_{2}}, \ldots, a_{p_{n}})$.
\end{definition}
In other words, $W(\mathcal{P})$ is the greatest common divisor of the weights of the edges in path $\mathcal{P}$.  Informally, we will refer to the GCD of the path $\mathcal{P}$.

\begin{definition}
Let $i, j$ be given, and let $P$ be the set of all paths between $i,j$.  We define $M(i,j) = [\{W(\mathcal{P})\}_{\mathcal{P} \in P}]$.
\end{definition}
In other words, given vertices $i, j$, $M(i,j)$ is the LCM of the GCDs of all paths between $i,j$.

Consequently:
\begin{theorem}
\label{theorem:GCD of LCM}
Let $(G, A)$ be an edge-weighted graph.  If $x = (x_{1}, x_{2}, \ldots, x_{n})$ is a spline in $S_{G}(A)$, then $x_{i} \equiv x_{j} \bmod M(i,j)$.
\end{theorem}
\begin{proof}
Let $P$ be the set of all paths between $i,j$, and let $\mathcal{P}$ be any path in $P$.  By Corollary \ref{corr:LCM of moduli}, $x_{i} \equiv x_{j} \bmod W(\mathcal{P})$.  Since this is true for all paths in $P$, then by Corollary \ref{ corr:GCD of moduli}, $x_{i} \equiv x_{j} \bmod M(i,j)$.
\end{proof}

We define the following:
\begin{definition}
Let $(G, A)$ be an edge-weighted graph, and let $x = (x_{1}, x_{2}, \ldots, x_{n})$ be a spline in $S_{G}(A)$.  Let $x_{i} = 0$ for one or more $i$.  Let $k$ be any vertex in $G$ with $x_{k} \neq 0$.  A \textbf{path to zero} is any path from $k$ to $i$, where $x_{j} \neq 0$ for any intermediate vertex.
\end{definition}

\begin{lemma}
Let $x$ be a spline in $S_{G}(A)$, and let $x_{i} = 0$ for at least one $i$.  If $x_{j} \neq 0$, then $x_{j} \equiv 0 \bmod P$, where $P$ is the Least Common Multiple of the Greatest Common Divisor of the edge weights along all paths to $0$ from $j$.
\end{lemma}
\begin{proof}
This follows immediately from Theorem \ref{theorem:GCD of LCM}.
\end{proof}
Of particular interest are splines whose first $k$ components are $0$.  We assume a collapse ordering $V$, and define:
\begin{definition}
The \textbf{flow up class} $\mathcal{F}_{k}$ is the set of splines in $S_{G}(A)$ where the first nonzero component is the $k+1$ component.
\end{definition}
It will be convenient to designate $\mathcal{F}_{0}$ to be the set of splines whose first component is non-zero.

Let $x$ be a spline in $\mathcal{F}_{k}$, and let $L(x)$ designate the leading (nonzero) component.  We say that $x$ is  \textbf{minimal} if, for any $y \in \mathcal{F}_{k}$, $\lvert L(x) \rvert \leq \lvert L(y) \rvert$.

Let $\mathcal{B} = \left\{B_{0}, B_{1}, B_{2}, \ldots, B_{n-1}\right\}$, where $B_{i} \in \mathcal{F}_{i}$ (so the first non-zero component of $B_{i}$ will be the $i+1$ component).  We now raise the question:  What elements $B_{i}$ form a minimal basis for $S_{G}(A)$?

We prove the following:
\begin{lemma}
\label{lemma star collapse invariant}
Let $i, j \in V$ be given, and let $(G', A')$ be a graph produced by a star deletion on $(G, A)$ that leaves vertices $i, j \in V'$.  Then $M(i,j)$, for paths in $(G, A)$, will equal $M(i,j)$ for paths in $(G', A')$.
\end{lemma}

\begin{proof}

Let $M$ be the set of GCDs of the edges along the paths from $i$ to $j$ in $(G, A)$, and $M'$ be the corresponding set for $(G', A')$.  

Let $\mathcal{P}$ be a path from $i$ to $j$ in $(G, A)$, and note that $W(\mathcal{P}) \in M$.  If $P$ does not include the deleted vertex, then $W(\mathcal{P})$ will be an element of $M'$, since a path in $(G, A)$ exists with the same edge weights.

On the other hand, suppose $\mathcal{P}$ passes through the deleted vertex, say along edges with weights $a, b$.  Then $W(\mathcal{P})$
Since the edges will be replaced with a single edge whose weight is the GCD of the incident edges,  weights incident on the vertex will be 



Let $W$ be the set of weights on $\mathcal{P}$.  Under star deletion, this path will become a new path; let $W'$ be the set of weights along this new path. The only difference between $W$ and $W'$ is that weights $p_{1}$, $p_{2}$ of the edges in $(G, A)$ joining to the deleted vertex will be replaced with a single edge with weight  $(p_{1}, p_{2})$.  But since $((a, b), c) = (a, b, c)$, it follows that the GCD of the weights in $W$ will be the same as the GCD of the weights in $W'$.  Hence $W(\mathcal{P})$ will also be an element of $M'$.

Thus $M \subset M'$.  

Consequently $M = M'$, and so the LCM of the elements of $M$ will also be the LCM of the elements of $M'$.  Thus if $M(i,j)$ is the LCM of the GCD of all paths from $i$ to $j$ in $(G, A)$, it remains the LCM of the GCD of all paths from $i$ to $j$ in $(G', A')$.
\end{proof}

Consequently:
\begin{theorem}
The minimal spline in $\mathcal{F}_{k}$ has leading term equal to the LCM of the GCD of all paths from $k + 1$ to zero.
\end{theorem}
\begin{proof}
Let $M$ be the LCM of the GCD of all paths from $k+1$ to zero in $(G, A)$.

By repeatedly applying star collapse on vertices $i > k + 1$, we obtain a graph $(G^{*}, A^{*})$ with vertices $1, 2, 3, \ldots, k + 1$ and edge set $E^{*}$.

The edges in $(G^{*}, A^{*})$ fall into one of two categories:  either they join vertices $i, j$ where $i, j \leq k$; or (without loss of generality) they join some vertex $i < k+1$ to vertex $j = k +1$.  

In the former case, $x_{i} = 0$, $x_{j} = 0$ solves the corresponding congruences.  The latter case gives a system of congruences of the form $x_{k+1} \equiv 0 \bmod a_{e}$, $e \in E^{*}$.  

Since star collapse does not alter the LCM of the GCD of the paths to zero, it follows that $x_{k+1} = M$ is the least positive solution to the system of congruences.  

We can then use Theorem \ref{theorem:  spline expansion} to find the remaining values $x_{k+2}$, $x_{k+3}, \ldots, $x_{n}$.  

\end{proof}



As an example, consider the graph in Figure \ref{fig:collapse0}, with collapse ordering $V = \left\{A, B, E, C, D\right\}$.  The minimal basis $\left\{B_{0}, B_{1}, B_{2}, B_{3}, B_{4}\right\}$ will be the following:

First, $B_{0} = (1, 1, 1, 1, 1)$, which will always be a basis vector for any $(G, A)$.

Next, let $x_{A} = 0$.  The second component of the basis vector will be the LCM of the GCD of the edge weights of all paths from $B$ to $A$.  We note there are the following paths:
\begin{itemize}
    \item 
    $B$ to $A$, with weight $8$ and GCD $8$,
    \item
    $B$ to $C$ to $A$, with edge weights $6, 9$ and 
    $(6, 9) = 3$,
    \item
    $B$ to $E$ to $A$, with edge weights $10, 14$ and $(10, 14) = 2$,
    \item
    $B$ to $C$ to $E$ to $A$, with edges weights $6, 3, 14$ and GCD $(6, 3, 14) = 1$.  (Hereafter we will simply list the edge weights in the GCD computation)
    \item
    $B$ to $D$ to $E$ to $A$, with GCD $(21, 9, 14) = 1$,
    \item
    $B$ to $D$ to $C$ to $A$, with GCD $(12, 9, 3, 9) = 3$
\end{itemize}
The GCD of the LCMs along these paths is $[8, 3, 2, 1, 1, 3] = 24$, so $L(B_{1}) = 24$.

Now let $x_{A}, x_{B} = 0$.  The third component of the basis vector $B_{2}$ will be the LCM of the GCD of  the edge weights of all paths from $E$ to either $A$ or $B$.  We note these paths are:
\begin{itemize}
    \item 
    $E$ to $A$, GCD $14$,
    \item
    $E$ to $B$, GCD $10$,
    \item
    $E$ to $C$ to $A$, GCD $(3, 9) = 3$,
    \item
    $E$ to $C$ to $B$, GCD $(3, 6) = 3$,
    \item
    $E$ to $D$ to $B$, GCD $(9, 12) = 3$,
\end{itemize}
The LCMs of these GCDs will be $[14, 10, 3, 3, 3] = 210$, so $L(B_{2}) = 210$.

Now let $x_{A}, x_{B}, x_{E} = 0$.  The fourth component of the basis vector $B_{3}$ will be the LCM of the GCD of  the edge weights of all paths from $C$ to $A, B$ or $E$.  We note that paths are:
\begin{itemize}
    \item 
    $C$ to $A$, GCD $9$,
    \item
    $C$ to $B$, GCD $6$,
    \item
    $C$ to $E$, GCD $3$,
\end{itemize}
The LCM of these GCDs will be $[9, 6, 3] = 18$, so $L(B_{3}) = 18$.

Finally let $x_{A}, x_{B}, x_{E}, x_{C} = 0$.  The fifth component of the basis vector $B_{4}$ will be the LCM of the GCD of the edge weights of all paths from $D$ to $A, B, E, C$; note that in fact the only paths to zero from $D$ are $D$ to $E$ (GCD $9$) and $D$ to $B$ (GCD $12)$, so the LCM of the GCDs will be $[9, 12] = 36$, and so $L(B_{4}) = 37$.

\section{New  Section:  Proof of Minimality}


We now prove an important result:
\begin{theorem}
The LCM of the GCD of all paths to $0$ from $v_{i}$ is invariant under a reduction operation.
\end{theorem}
\begin{proof}
There are two reduction operations, so we will consider them separately.

Let $\mathcal{P} = \left\{p_{1}, p_{2}, \ldots, p_{n}\right\}$ be the set of all paths to $0$ from vertex $i$, and let 
\end{proof}

